Game theory on the blockchain: a model for games with smart contracts

We propose a model for games in which the players have shared access to a blockchain that allows them to deploy smart contracts to act on their behalf. This changes fundamental game-theoretic assumptions about rationality since a contract can commit a player to act irrationally in specific subgames, making credible otherwise non-credible threats. This is further complicated by considering the interaction between multiple contracts which can reason about each other. This changes the nature of the game in a nontrivial way as choosing which contract to play can itself be considered a move in the game. Our model generalizes known notions of equilibria, with a single contract being equivalent to a Stackelberg equilibrium, and two contracts being equivalent to a reverse Stackelberg equilibrium. We prove a number of bounds on the complexity of computing SPE in such games with smart contracts. We show that computing an SPE is $\textsf{PSPACE}$-hard in the general case. Specifically, in games with $k$ contracts, we show that computing an SPE is $\Sigma_k^\textsf{P}$-hard for games of imperfect information. We show that computing an SPE remains $\textsf{PSPACE}$-hard in games of perfect information if we allow for an unbounded number of contracts. We give an algorithm for computing an SPE in two-contract games of perfect information that runs in time $O(m\ell)$ where $m$ is the size of the game tree and $\ell$ is the number of terminal nodes. Finally, we conjecture the problem to be $\textsf{NP}$-complete for three contracts.

==> preamble_contracts.tex <==
\usepackage{adjustbox}
\usepackage{amsmath,amssymb}
\usepackage{mathrsfs}
\usepackage{framed}
\usepackage{booktabs}
\usepackage{algorithmic}
\usepackage{bbm}
\usepackage{xcolor}
\usepackage{hyperref}
\usepackage[inline,shortlabels]{enumitem}
\usepackage[ruled,vlined]{algorithm2e}
\usepackage[capitalise,nameinlink]{cleveref}
\usepackage{todonotes}

\usepackage{tikz}
\usepackage{tikz-qtree}

\usetikzlibrary{calc}
\usetikzlibrary{trees}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{arrows.meta}

\input{macros}

\hypersetup{nolinks=true}

\newcommand{\inducible}[0]{\mathscr{R}}
\newcommand{\util}{\textsf{util}}
\newcommand{\coloring}{\textsc{3-coloring}}
\newcommand{\owner}{\textsf{owner}}
% \usepackage[colorinlistoftodos]{todonotes}

% Used for algo. formatting
\usepackage[ruled,vlined]{algorithm2e}

\renewcommand{\log}{\lg}

\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\eps}{\varepsilon}
\newcommand{\Flazy}{\F}
\newcommand{\bigO}{\widetilde{O}}

\newcommand{\bTree}{\mathcal{T}}

\DeclareMathOperator{\depth}{depth}

\DeclareMathOperator{\negl}{negl}
\DeclareMathOperator{\op}{op}
\DeclareMathOperator{\data}{data}
\DeclareMathOperator{\addr}{a}
\DeclareMathOperator{\rd}{read}
\DeclareMathOperator{\wri}{write}
\DeclareMathOperator{\IP}{IP}

\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

\DeclareMathOperator{\HH}{H}
\DeclareMathOperator{\comp}{\,\diamond\,}
\DeclareMathOperator{\given}{\,\vert\,}

\DeclareMathOperator{\view}{view}
\DeclareMathOperator{\simu}{sim}

\newcommand{\zo}{\{ 0, 1\}}
\newcommand{\poly}{\operatorname{poly}}
\renewcommand{\P}{\mathsf{P}}
\newcommand{\Q}{\mathsf{Q}}
\newcommand{\F}{\mathsf{F}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\Pcolor}{P_\text{color}}
\newcommand{\Pcheck}{P_\text{check}}

\newcommand{\player}[0]{P}
\newcommand{\playern}[1]{\player_{#1}}

\newcommand{\gamepath}[0]{\mathfrak{p}} % consists of moves by players, needs better name
\newcommand{\subgame}[0]{G_s} % needs better name

\newcommand{\subgameA}[1]{\subgame(#1)}

\newcommand{\utility}[0]{u}

\newcommand{\moveplayer}[1]{\ensuremath{\text{P}(#1)}} % takes a move in the tree and returns the player

\newcommand{\gametree}[0]{T}
\newcommand{\cut}[0]{c}
\newcommand{\cutof}[1]{\ensuremath{c^{(#1)}}}

% player leader/follower
\newcommand{\playerL}[0]{\playerA}
\newcommand{\playerF}[0]{\playerB}

% when you just need some players
\newcommand{\playerA}[0]{\playern{1}}
\newcommand{\playerB}[0]{\playern{2}}

\newcommand{\EXP}{\textsf{EXP}}

\def\btc{}

% \def\btc{\leavevmode
%  {\setbox0=\hbox{\textsf{B}}%
%    \dimen0\ht0 \advance\dimen0 0.2ex
%    \ooalign{\hfil \box0\hfil\cr
%      \hfil\vrule height \dimen0 depth.2ex\hfil\cr
%    }%
%  }%
% }

\newcommand{\prob}[3]{\begin{framed}\vspace{-0.5cm}
    \begin{center}
        \textsf{#1}
    \end{center}\vspace{-0.6cm}\hrulefill\\
    \noindent \textbf{Instance}: \,#2\\
    \noindent \textbf{Question}: #3\vspace{-0.1cm}
\end{framed}}

\newcommand{\mA}{\mathcal{A}}

\newcommand{\SD}{\operatorname{D}}

\renewcommand{\H}{\operatorname{H}}

\newcommand{\PSPACE}{\textsf{PSPACE}}
\renewcommand{\P}{\textsf{P}}
\newcommand{\NAND}{\textsf{NAND}}
\newcommand{\NP}{\textsf{NP}}

